WeNet: Production oriented Streaming and Non-streaming End-to-End Speech Recognition Toolkit

In this paper, we propose an open source, production first, and production ready speech recognition toolkit called WeNet in which a new two-pass approach is implemented to unify streaming and non-streaming end-to-end (E2E) speech recognition in a single model. The main motivation of WeNet is to close the gap between the research and the production of E2E speechrecognition models. WeNet provides an efficient way to ship ASR applications in several real-world scenarios, which is the main difference and advantage to other open source E2E speech recognition toolkits. In our toolkit, a new two-pass method is implemented. Our method propose a dynamic chunk-based attention strategy of the the transformer layers to allow arbitrary right context length modifies in hybrid CTC/attention architecture. The inference latency could be easily controlled by only changing the chunk size. The CTC hypotheses are then rescored by the attention decoder to get the final result. Our experiments on the AISHELL-1 dataset using WeNet show that, our model achieves 5.03\% relative character error rate (CER) reduction in non-streaming ASR compared to a standard non-streaming transformer. After model quantification, our model perform reasonable RTF and latency.

==> IEEEtran/tools/README <==

January 11, 2007


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.
 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later
 3. the IEEE itemize, enumerate and description list environments
 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

IEEEtrantools.sty should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
1/2007 V1.2 (V1.7 of IEEEtran.cls) changes:

 1. Several commands and enviroments have depreciated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow use of the
    obsolete forms, but with an warning message to the console during
    compilation:
    \IEEEPARstart
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
 
 2. These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. \normalsizebaselineskip no longer provided. 

 4. New \IEEEPARstart controls:
    \IEEEPARstartHEIGHTTEXT, \IEEEPARstartFONTSTYLE, \IEEEPARstartCAPSTYLE,
    \IEEEPARstartWORDFONTSTYLE, \IEEEPARstartWORDCAPSTYLE,
    \IEEEPARstartHOFFSET, \IEEEPARstartITLCORRECT
    and the (output) length \IEEEPARstartletwidth.

 5. Provide for an optional argument to \bstctlcite to provide a way to
    specify a different aux file. Define \bstctlcite even if it has already
    been defined.

********************************** Files **********************************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************



==> source/02related.tex <==
\section{Related Works}

% Espnet
Espnet is the most popular open source platform which mainly focuses on end-to-end ASR and adopts widely used dynamic neural network toolkits Chainer and PyTorch as the main deep learning engine. Espnet is useful and widely-used for research, but the application support of streaming scene is insufficient. Besides it is hard to directly use the model trained by Espnet in production, and there is no production consideration or support in Espnet design. As far as above concerned, there is no such toolkit that focuses on production oriented E2E speech recognition currently.

% RNN-T two pass

% Two pass based model~\cite{sainath2019two}  was proposed on RNN-T and achieves comparable accuracy to a LAS model. 
% However, RNN-T training is very memory consuming~\cite{li2019improving} so that we can not use a large batch for training on typical GPUs, which results in a very slow training speed as well as poor performance. Besides, RNN-T training is also unstable. CTC pre-training  ~\cite{rao2017exploring} and \textit{Cross Entropy}(CE) pre-training were proposed in ~\cite{hu2020exploring} to assist RNN-T training, while pre-training was also tricky and complicated. These increase the difficulty of using RNN-T in speech recognition application, especially when lacking computing and research resources.
% And it was pointed out that training directly from scratch is unstable using combined RNN-T loss and LAS loss, so a three-step training strategy was proposed in ~\cite{sainath2019two} to solve the problem, which further complicates the training pipeline.

% % Model-Y and Universal ASR
% For unified non-streaming and streaming model,
% Y-model uses variable context at training and several optional contexts at inference. However, the optional contexts are predefined at the training stage, and the contexts have to be carefully designed in terms of the number of encoder layers, the kernel size of the convolution operation.
% Moreover dual-mode only has one streaming configuration in both training and inference. If we want another streaming model with different latency at inference, the model needs to be totally retrained. Besides, both Y-model and dual-mode are RNN-T based models. They have the same drawbacks as RNN-T.

% Our proposed U2, a CTC-AED joint model, is trained by combined CTC and AED loss and dynamic chunk attention. It not only unifies the non-streaming and streaming model, giving promising result, but also significantly simplifies the training pipeline, as well as dynamically controls the trade-off between latency and accuracy in streaming applications.

